A Generative Security Application Engineering Curriculum

Generative AI and large language models (LLMs) are transforming security by automating many tasks being performed manually. With such automation changing the practice of security as we know it, it is imperative that we prepare future students for the technology landscape they will ultimately face. Towards this end, we describe an initial curriculum and course that attempts to show students how to apply generative AI in order to solve problems in security. By refocusing security education and training on aspects uniquely suited for humans and showing students how to leverage automation for the rest, we believe we can better align security education practices with generative AI as it evolves.

==> acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> acmart-master/README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

==> macro.tex <==
% @device(postscript)
% @style(size = 11)
% @style(spacing 1.5)
% @begin{format}

\def \A {{\cal A}}
\def \B {{\cal B }}
\def \C {{\cal C }}
\def \D {{\cal D}}
\def \E {{\cal E}}
\def \F {{\cal F}}
\def \I {{\cal I}}
\def \J {{\cal J}}
\def \K {{\cal K}}
\def \L {{\cal L}}
\def \M {{\cal M}}
\def \O {{\cal O}}
\def \P {{\cal P}}
\def \R {{\cal R}}
\def \S {{\cal S}}
\def \T {{\cal T }}

\def \alph {{\bar \alpha}}
\def \bsigma {\bar\sigma}
\def \hsigma {\hat\sigma}
\def \sqsigma {\tilde\sigma}

%
\def \eps {\epsilon}
\def \etc {\it etc.\ }
%\def \example {\noindent {\bf Example\ }}
\def \ie {{\it i.e.,}}
\def \eg {e.g.,}

\def \Reals {R\kern -0.82 em R\ }
\def \Timeinf {N\kern -0.82 em N^\infty}
\def \Timeint {N\kern -0.82 em N^{\infty} \times N\kern -0.82 em N^{\infty}}
\def \Time {N\kern -0.82 em N}
\def \notintr {\intr\kern -.8 em / \ }

\def \necc {\hbox to 0pt {\sqcup\hss} \sqcap}
\def \notexists {\exists\kern -.4 em / }
\def \notin {\in\kern -.8 em / }

\def \qed {\hfill{\boxit{\null}{3pt}{3pt}}\vspace*{5pt}}
%\def \qed {}
\def \proof {\noindent {\bf Proof:\quad}}
\def \endproof{\qed}

\def \la {\langle}
\def \ra {\rangle}
\def \precedes {\longrightarrow}
\def \infeasible {\ominus}
\def \concurrent {\parallel}
\def \defined {\stackrel{\rm def}{=}}
\def \st {\hspace*{-1pt}::}
\def \implies {\mbox{$\Rightarrow$}}


\newcommand{\seq}[1]{\mbox{$\la #1 \ra$}}
\newcommand{\oprule}[2] {\begin{array}{c}
                         #1 \\ \hline
                         #2 \end{array}}
\newcommand{\oprulecond}[3] {\begin{array}{rl}
                              {\begin{array}{c}
                               #1 \\ \hline
                               #2 \end{array}}& #3
                            \end{array}}

\def \meanop #1{{\bf O}\lsem #1 \rsem}

\def\Month{\ifcase\month xxx\or January\or February\or March\or April\or
           May\or  June\or July\or August\or September\or
           October\or November\or December\else zzz\fi}

\def\boxit#1#2#3{\vbox{\hrule
  \hbox{\vrule\hskip#2\vbox{\vskip#3{#1}\vskip#3}\hskip#2\vrule}\hrule}}

\def\beginlmath{\relax\ifmmode\@badmath\else\begin{trivlist}\item[]\leavevmode
 \hbox to\linewidth\bgroup$ \displaystyle
 \hskip\mathindent\bgroup\fi}
%
\def\endlmath{\relax\ifmmode \egroup $\hfil \egroup \end{trivlist}\else \@badmath \fi}
\newdimen\mathindent
\mathindent = \leftmargini

\newcommand{\nonterm}[1] {$\la$#1$\ra$}

\long\def \ignoreme#1{}

\def \After {{\bf after}}
\def \Begin {{\bf Begin}}
\def \By {{\bf by}}
\def \Case {{\bf Case}}
\def \Delay {{\bf delay}}
\def \Do  {{\bf do}}
\def \Each {{\bf each}}
\def \Else {{\bf else}}
\def \Elseif {{\bf else if}}
\def \End  {{\bf End}}
\def \Endcase {{\bf end}}
\def \Endif {{\bf endif}}
\def \Endfor {{\bf end}}
\def \Endwhile {{\bf end}}
\def \Every {{\bf every}}
\def \Finish {{\bf finish}}
\def \For {{\bf for}}
\def \Foreach {{\bf foreach}}
\def \If  {{\bf if}}
\def \Loop {{\bf loop}}
\def \Od  {{\bf od}}
\def \Receive {{\bf receive}}
\def \Send  {{\bf send}}
\def \Skip  {{\bf skip}}
\def \Start {{\bf start}}
\def \Then {{\bf then}}
\def \To   {{\bf to}}
\def \While {{\bf while}}
\def \Within {{\bf within}}
\def \Wait {{\bf wait}}

%%\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{problem}{Problem}[section]
\newtheorem{define}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{fact}{Fact}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{remark}{Remark}[section]
%\newtheorem{algorithm}{Algorithm}[section]
%\def\floor#1{\lfloor #1\rfloor} %  floor and ceiling (from math mode)
\def\floor#1{\left\lfloor #1\right\rfloor}
%\def\ceil#1{\lceil #1\rceil}
\def\ceil#1{\left\lceil #1\right\rceil}
\def\first#1{\left( #1\right)}
\def\second#1{\left\{ #1\right\}}
\def\third#1{\left[ #1\right]}
\def\ang#1{\langle #1\rangle}   %  angle brackets <...>

\marginparwidth=0.50in
\newcommand\mnote{\marginpar{\Large $\leftarrow$}}


\newcommand\doublespace{\renewcommand\baselinestretch{1.5}}
\newcommand\singlespace{\renewcommand\baselinestretch{1.05}}
\newcommand\myspacing{\renewcommand\baselinestretch{1.3}}
\newcommand\smallspacing{\renewcommand\baselinestretch{1.1}}
\smallspacing


\newenvironment{algorithm}[1]{\begin{tabbing}
****\=****\=****\=****\=****\=****\=****\=\kill
{\bf Algorithm #1} \\[5pt]}{\end{tabbing}}

\newenvironment{program}{\begin{tabbing}
****\=****\=****\=****\=****\=****\=****\=\kill \\
}{\end{tabbing}}

%\input fancybox.sty

\newlength{\mylength}
\fboxsep=0.8cm

\newenvironment{FramedTable}[1]%
{\begin{table}[#1]
  \begin{center}%
  \begin{Sbox}%
      \setlength{\mylength}{\textwidth}%
      \addtolength{\mylength}{-2\fboxsep}%
      \addtolength{\mylength}{-2\fboxrule}%
      \begin{minipage}{.8\mylength}}%
        {\end{minipage}\end{Sbox}\doublebox{\TheSbox}\end{center}\end{table}}%

\newenvironment{FramedFigure}%
{\begin{figure}[thb]
  \begin{center}%
  \begin{Sbox}%
      \setlength{\mylength}{\textwidth}%
      \addtolength{\mylength}{-2\fboxsep}%
      \addtolength{\mylength}{-2\fboxrule}%
      \begin{minipage}{.8\mylength}}%
        {\end{minipage}\end{Sbox}\doublebox{\TheSbox}\end{center}\end{figure}}%

\newenvironment{fminipage}%
{\begin{Sbox}\begin{minipage}}%
{\end{minipage}\end{Sbox}\doublebox{\TheSbox}}


%---------------------------------------------------
% My enumerate environment
%

\newcounter{step}
\newcounter{estep}
\def\Enumerate{
\setcounter{estep}{1}
\begin{list}
{(\arabic{estep})}
{\usecounter{estep}\setlength{\parsep}{3pt}\setlength{\itemsep}{0pt}}
}
\def\endEnumerate{\end{list}}
%---------------------------------------------------
\newcounter{case}
\def\Cases{
\setcounter{case}{1}
\begin{list}
{{\bf Case \arabic{case}:}}
{\usecounter{case}\setlength{\parsep}{0pt}\setlength{\itemsep}{2pt}
                \setlength{\labelwidth}{15pt}\setlength{\leftmargin}{40pt}}
}
\def\endCases{\end{list}}
%
%---------------------------------------------------

%---------------------------------------------------
% Algorithm environment
%
\def\mytab{
 \begin{tabbing}
 123 \= 123 \= 123 \= 123 123 \= \kill
 }
\def\endmytab{\end{tabbing}}
%

%---------------------------------------------------
% Algorithm environment
%
\def\steps{
\setcounter{step}{1}
\begin{list}
{{\bf Step \arabic{step}}}
{\usecounter{step}\setlength{\parsep}{0pt}\setlength{\itemsep}{2pt}
                \setlength{\labelwidth}{15pt}\setlength{\leftmargin}{40pt}}
}
\def\endsteps{\end{list}}
%
%---------------------------------------------------


\newcounter{subsubsubsection}
\newcommand{\subsubsubsection}[1]{\addtocounter{subsubsubsection}{1} \paragraph{\thesubsubsection.\thesubsubsubsection\ #1}}

\newcommand{\eoe}{\hfill $\Diamond$ \paragraph{}}

\newcommand{\concat}{\,||\,}
\newcommand{\bits}{\{0,1\}}
\newcommand{\xor}{\oplus}

